A Sufficient Statistic for Influence in Structured Multiagent Environments

Making decisions in complex environments is a key challenge in artificial intelligence (AI). Situations involving multiple decision makers are particularly complex, leading to computational intractability of principled solution methods. A body of work in AI has tried to mitigate this problem by trying to distill interaction to its essence: how does the policy of one agent influence another agent? If we can find more compact representations of such influence, this can help us deal with the complexity, for instance by searching the space of influences rather than the space of policies. However, so far these notions of influence have been restricted in their applicability to special cases of interaction. In this paper we formalize influence-based abstraction (IBA), which facilitates the elimination of latent state factors without any loss in value, for a very general class of problems described as factored partially observable stochastic games (fPOSGs). On the one hand, this generalizes existing descriptions of influence, and thus can serve as the foundation for improvements in scalability and other insights in decision making in complex multiagent settings. On the other hand, since the presence of other agents can be seen as a generalization of single agent settings, our formulation of IBA also provides a sufficient statistic for decision making under abstraction for a single agent. We also give a detailed discussion of the relations to such previous works, identifying new insights and interpretations of these approaches. In these ways, this paper deepens our understanding of abstraction in a wide range of sequential decision making settings, providing the basis for new approaches and algorithms for a large class of problems.

==> figs/frag_br_ag2.tex <==
\scriptsize
\psfrag{t0}[cc][cc]{   $t=0$    }
\psfrag{t1}[cc][cc]{   $t=1$    }
\psfrag{t2}[cc][cc]{   $t=2$    }
\psfrag{t_h}[cc][cc]{  $\substack{\text{terminal stage} \\  (t=3=h)}$  }
%
%-state factors-
%t=0
\psfrag{x10}[cc][cB]{  $\sfacI {1} $ }
\psfrag{x20}[cc][cB]{  $\sfacI {2} $ }
\psfrag{x30}[cc][cB]{  $\sfacI {3} $ }
\psfrag{x40}[cc][cB]{  $\sfacI {4} $ }
%t=1
\psfrag{x11}[cc][cB]{  $\sfacI {1} $ }
\psfrag{x21}[cc][cB]{  $\sfacI {2} $ }
\psfrag{x31}[cc][cB]{  $\sfacI {3} $ }
\psfrag{x41}[cc][cB]{  $\sfacI {4} $ }
%t=2
\psfrag{x12}[cc][cB]{  $\sfacI {1} $ }
\psfrag{x22}[cc][cB]{  $\sfacI {2} $ }
\psfrag{x32}[cc][cB]{  $\sfacI {3} $ }
\psfrag{x42}[cc][cB]{  $\sfacI {4} $ }
%t=3
\psfrag{x13}[cc][cB]{  $\sfacI {1} $ }
\psfrag{x23}[cc][cB]{  $\sfacI {2} $ }
\psfrag{x33}[cc][cB]{  $\sfacI {3} $ }
\psfrag{x43}[cc][cB]{  $\sfacI {4} $ }
%
%-actions-
%t=0
\psfrag{a10}[cc][cB]{  $\aAT {1} {0} $ }
\psfrag{a20}[cc][cB]{  $\aAT {2} {0} $ }
%t=1
\psfrag{a11}[cc][cB]{  $\aAT {1} {1} $ }
\psfrag{a21}[cc][cB]{  $\aAT {2} {1} $ }
%t=2
\psfrag{a12}[cc][cB]{  $\aAT {1} {2} $ }
\psfrag{a22}[cc][cB]{  $\aAT {2} {2} $ }
%-observations-
%t=0
\psfrag{o10}[cc][cB]{  $\aoHistAT {1} {0} $ }
\psfrag{o20}[cc][cB]{  $\oAT {2} {0} $ }
%t=1
\psfrag{o11}[cc][cB]{  $\aoHistAT {1} {1} $ }
\psfrag{o21}[cc][cB]{  $\oAT {2} {1} $ }
%t=2
\psfrag{o12}[cc][cB]{  $\aoHistAT {1} {2} $ }
\psfrag{o22}[cc][cB]{  $\oAT {2} {2} $ }
%-rewards-
%t=0
\psfrag{r10}[cc][cB]{  $\rAT {1} {0} $ }
\psfrag{r20}[cc][cB]{  $\rAT {2} {0} $ }
%t=1
\psfrag{r11}[cc][cB]{  $\rAT {1} {1} $ }
\psfrag{r21}[cc][cB]{  $\rAT {2} {1} $ }
%t=2
\psfrag{r12}[cc][cB]{  $\rAT {1} {2} $ }
\psfrag{r22}[cc][cB]{  $\rAT {2} {2} $ }


==> figs/frag_cf.tex <==
\scriptsize
\psfrag{t0}[cc][cc]{   $t=0$    }
\psfrag{t1}[cc][cc]{   $t=1$    }
%\psfrag{t2}[cc][cc]{   $t=2$    }
\psfrag{t2}[cc][cc]{  $\substack{\text{terminal stage} \\  (t=2=h)}$  }
%
%-state factors-
%t=0
%\psfrag{x10}[cc][cB]{  $\sfacIT {1} {0} $ }
%\psfrag{x20}[cc][cB]{  $\sfacIT {2} {0} $ }
%\psfrag{x30}[cc][cB]{  $\sfacIT {3} {0} $ }
%\psfrag{x40}[cc][cB]{  $\sfacIT {4} {0} $ }
%%t=1
%\psfrag{x11}[cc][cB]{  $\sfacIT {1} {1} $ }
%\psfrag{x21}[cc][cB]{  $\sfacIT {2} {1} $ }
%\psfrag{x31}[cc][cB]{  $\sfacIT {3} {1} $ }
%\psfrag{x41}[cc][cB]{  $\sfacIT {4} {1} $ }
%%t=2
%\psfrag{x12}[cc][cB]{  $\sfacIT {1} {2} $ }
%\psfrag{x22}[cc][cB]{  $\sfacIT {2} {2} $ }
%\psfrag{x32}[cc][cB]{  $\sfacIT {3} {2} $ }
%\psfrag{x42}[cc][cB]{  $\sfacIT {4} {2} $ }
%%t=3
%\psfrag{x13}[cc][cB]{  $\sfacIT {1} {3} $ }
%\psfrag{x23}[cc][cB]{  $\sfacIT {2} {3} $ }
%\psfrag{x33}[cc][cB]{  $\sfacIT {3} {3} $ }
%\psfrag{x43}[cc][cB]{  $\sfacIT {4} {3} $ }
%-state factors-
%t=0
\psfrag{x10}[cc][cB]{  $\sfacI {1}  $ }
\psfrag{x20}[cc][cB]{  $\sfacI {2}  $ }
\psfrag{x30}[cc][cB]{  $\sfacI {3}  $ }
\psfrag{x40}[cc][cB]{  $\sfacI {4}  $ }
%t=1
\psfrag{x11}[cc][cB]{  $\sfacI {1}  $ }
\psfrag{x21}[cc][cB]{  $\sfacI {2}  $ }
\psfrag{x31}[cc][cB]{  $\sfacI {3}  $ }
\psfrag{x41}[cc][cB]{  $\sfacI {4}  $ }
%t=2
\psfrag{x12}[cc][cB]{  $\sfacI {1}  $ }
\psfrag{x22}[cc][cB]{  $\sfacI {2}  $ }
\psfrag{x32}[cc][cB]{  $\sfacI {3}  $ }
\psfrag{x42}[cc][cB]{  $\sfacI {4}  $ }
%t=3
\psfrag{x13}[cc][cB]{  $\sfacI {1}  $ }
\psfrag{x23}[cc][cB]{  $\sfacI {2}  $ }
\psfrag{x33}[cc][cB]{  $\sfacI {3}  $ }
\psfrag{x43}[cc][cB]{  $\sfacI {4}  $ }
%
%-actions-
%t=0
%\psfrag{a10}[cc][cB]{  $\aAT {1} {0} $ }
%\psfrag{a20}[cc][cB]{  $\aAT {2} {0} $ }
%%t=1
%\psfrag{a11}[cc][cB]{  $\aAT {1} {1} $ }
%\psfrag{a21}[cc][cB]{  $\aAT {2} {1} $ }
%%t=2
%\psfrag{a12}[cc][cB]{  $\aAT {1} {2} $ }
%\psfrag{a22}[cc][cB]{  $\aAT {2} {2} $ }
\psfrag{a10}[cc][cB]{  $\aA {1}  $ }
\psfrag{a20}[cc][cB]{  $\aA {2}  $ }
%t=1
\psfrag{a11}[cc][cB]{  $\aA {1}  $ }
\psfrag{a21}[cc][cB]{  $\aA {2}  $ }
%t=2
\psfrag{a12}[cc][cB]{  $\aA {1}  $ }
\psfrag{a22}[cc][cB]{  $\aA {2}  $ }
%
%
%-observations-
%t=0
%\psfrag{o10}[cc][cB]{  $\oAT {1} {0} $ }
%\psfrag{o20}[cc][cB]{  $\oAT {2} {0} $ }
%%t=1
%\psfrag{o11}[cc][cB]{  $\oAT {1} {1} $ }
%\psfrag{o21}[cc][cB]{  $\oAT {2} {1} $ }
%%t=2
%\psfrag{o12}[cc][cB]{  $\oAT {1} {2} $ }
%\psfrag{o22}[cc][cB]{  $\oAT {2} {2} $ }
%t=0
\psfrag{o10}[cc][cB]{  $\oA {1} $ }
\psfrag{o20}[cc][cB]{  $\oA {2} $ }
%t=1
\psfrag{o11}[cc][cB]{  $\oA {1} $ }
\psfrag{o21}[cc][cB]{  $\oA {2} $ }
%t=2
\psfrag{o12}[cc][cB]{  $\oA {1} $ }
\psfrag{o22}[cc][cB]{  $\oA {2} $ }
%\tiny
%-rewards-
%t=0
%\psfrag{r10}[cc][cB]{  $\rAT {1} {0} $ }
%\psfrag{r20}[cc][cB]{  $\rAT {2} {0} $ }
%%t=1
%\psfrag{r11}[cc][cB]{  $\rAT {1} {1} $ }
%\psfrag{r21}[cc][cB]{  $\rAT {2} {1} $ }
%%t=2
%\psfrag{r12}[cc][cB]{  $\rAT {1} {2} $ }
%\psfrag{r22}[cc][cB]{  $\rAT {2} {2} $ }
\psfrag{r10}[cc][cB]{  $\rA {1} $ }
\psfrag{r20}[cc][cB]{  $\rA {2} $ }
%t=1
\psfrag{r11}[cc][cB]{  $\rA {1} $ }
\psfrag{r21}[cc][cB]{  $\rA {2} $ }
%t=2
\psfrag{r12}[cc][cB]{  $\rA {1} $ }
\psfrag{r22}[cc][cB]{  $\rA {2} $ }


==> figs/frag_cf_dectig.tex <==
%t=0
%\psfrag{tl0}[cc][cB]{  $\argsT{\text{tiger}}{0} $ }
%\psfrag{j0}[cc][cB] {  $\argsT{\text{pja}}  {0} $ }
%%t=1
%\psfrag{tl1}[cc][cB]{  $\argsT{\text{tiger}}{1} $ }
%\psfrag{j1}[cc][cB] {  $\argsT{\text{pja}}  {1} $ }
%%t=2
%\psfrag{tl2}[cc][cB]{  $\argsT{\text{tiger}}{2} $ }
%\psfrag{j2}[cc][cB] {  $\argsT{\text{pja}}  {2} $ }
%%t=3
%\psfrag{tl3}[cc][cB]{  $\argsT{\text{tiger}}{3} $ }
%\psfrag{j3}[cc][cB] {  $\argsT{\text{pja}}  {3} $ }
%t=0
\tiny
\psfrag{tl0}[cc][cB]{  $\text{tiger} $ }
\psfrag{j0}[cc][cB] {  $\text{pja}  $ }
%t=1
\psfrag{tl1}[cc][cB]{  $\text{tiger} $ }
\psfrag{j1}[cc][cB] {  $\text{pja}  $ }
%t=2
\psfrag{tl2}[cc][cB]{  $\text{tiger} $ }
\psfrag{j2}[cc][cB] {  $\text{pja}  $ }
%t=3
\psfrag{tl3}[cc][cB]{  $\text{tiger} $ }
\psfrag{j3}[cc][cB] {  $\text{pja}  $ }


==> macros.tex <==
\global\long\def\discount{\gamma}%

\global\long\def\ts{t}%

\global\long\def\s{s}%

\global\long\def\sT#1{{\argsT{s}{#1}}}%

\global\long\def\Aug#1{\bar{{#1}}}%

\global\long\def\sAugAT#1#2{{\argsAT{\Aug{\s}}{#1}{#2}}}%

\global\long\def\excl#1{-{#1}}%

\global\long\def\sAugA#1{{\argsA{\bar{s}}{#1}}{}}%

\global\long\def\sAugAT#1#2{{\argsAT{\bar{s}}{#1}{#2}}}%

\global\long\def\aHistAT#1#2{{\argsAT{\AH}{#1}{\,#2}}}%

\global\long\def\oHistAT#1#2{{\argsAT{\OH}{#1}{\,#2}}}%

\global\long\def\aoHistAT#1#2{{\argsAT{\AOH}{#1}{#2}}}%

\global\long\def\aoHistGT#1#2{{\argsGT{\AOH}{#1}{#2}}}%

\global\long\def\aA#1{{\argsA{a}{#1}}}%

\global\long\def\aAT#1#2{{\argsAT{a}{#1}{#2}}}%

\global\long\def\oA#1{{\argsA{o}{#1}}}%

\global\long\def\oAT#1#2{{\argsAT{o}{#1}{#2}}}%

\global\long\def\ja{{\joint{\lyxmathsym{\AC}}}}%

\global\long\def\jaT#1{{\argsT{\ja}{#1}}}%

\global\long\def\jaG#1{{\argsG{\lyxmathsym{\AC}}{#1}}}%

\global\long\def\jaGT#1#2{{\argsGT{\lyxmathsym{\AC}}{#1}{#2}}}%

\global\long\def\joT#1{{\argsT{\jo}{#1}}}%

\global\long\def\joGT#1#2{{\argsGT{\OB}{#1}{#2}}}%

\global\long\def\polA#1{\argsA{\POL}{#1}}%

\global\long\def\drAT#1#2{\argsAT{\DR}{#1}{#2}}%

\global\long\def\jdrGT#1#2{\argsAT{\joint\DR}{#1}{#2}}%

\global\long\def\pPolAT#1#2{\argsAT{\pP}{#1}{#2}}%

\global\long\def\pJPolGT#1#2{\argsAT{\joint\pP}{#1}{#2}}%

\global\long\def\jpolG#1{\argsG{\joint{\POL}}{#1}}%

\global\long\def\bA#1{\argsA{b}{#1}}%

\global\long\def\bO{{b^{0}}}%

\global\long\def\lbA#1{\argsAT{b}{#1}{l}}%
\begin{comment}
local-form belief
\end{comment}

\global\long\def\gbA#1{\argsAT{b}{#1}{g}}%
\begin{comment}
global-form belief
\end{comment}

\global\long\def\RA#1{\argsA{R}{#1}}%

\global\long\def\V{V}%

\global\long\def\Q{Q}%

\global\long\def\QT#1{\argsT{Q}{#1}}%

\global\long\def\nmfA#1{\argsA{\joint\NMF}{#1}}%

\global\long\def\nmfAT#1#2{\argsAT{\joint\NMF}{#1}{#2}}%

\global\long\def\nmfI#1{\argsI{\NMF}{#1}}%

\global\long\def\nmfIT#1#2{\argsIT{\NMF}{#1}{#2}}%

\global\long\def\mfA#1{{\argsA{\joint\MF}{#1}}}%

\global\long\def\mfAT#1#2{{\argsAT{\joint\MF}{#1}{#2}}}%

\global\long\def\mfI#1{{\argsI{\MF}{#1}}}%

\global\long\def\mflAT#1#2{{\argsAT{\joint\MFl}{#1}{#2}}}%

\global\long\def\mflI#1{{\argsI{\MFl}{#1}}}%

\global\long\def\mflIT#1#2{{\argsIT{\MFl}{#1}{#2}}}%

\global\long\def\mfnAT#1#2{{\argsAT{\joint\MFn}{#1}{#2}}}%

\global\long\def\mfnI#1{{\argsI{\MFn}{#1}}}%

\global\long\def\mfnIT#1#2{{\argsIT{\MFn}{#1}{#2}}}%

\global\long\def\dHistAT#1#2{\vec{\DSET}\argsAT{}{#1}{#2}}%

\global\long\def\dsetAT#1#2{\DSET\argsAT{}{#1}{#2}}%

\global\long\def\iffunc{I}%

\global\long\def\ifsGT#1#2{\argsGT{u}{#1}{#2}}%

\global\long\def\ifsAT#1#2{\argsAT{u}{#1}{#2}}%

\global\long\def\ifpiAT#1#2{\argsAT{I}{\rightarrow#1}{#2}}%

\global\long\def\pfA#1{\argsA{\joint\PF}{#1}}%

\global\long\def\pfAT#1#2{\argsAT{\joint\PF}{#1}{#2}}%



==> preamble.natbib-emul.tex <==

\makeatletter
%emulate natbib commands using 'theapa' backend (for JAIR)
%
%\usepackage{twoopt}
%\newcommandtwoopt{\citep}[3][][]{WRITING cite\textless#1\textgreater[#2]\{\detokenize{#3}\} \cite<#1>[#2]{#3}}
%
%\newcommand{\citep}[2][hello]{WRITING cite[#1]\{\detokenize{#2}\} \cite[#1]{#2}}
%\newcommand{\citep}[2][]   {\cite[#1]{#2}}

%---
%make sure not to put any spaces here:
\def\ifempty#1{\def\temp{#1}\ifx\temp\empty}
%\def \mymacro#1{ \ifempty{#1} empty \else not empty \fi }
%\mymacro{something} % prints "not empty"
%\mymacro{}          % prints "empty"
%---
\def\citep{%
  %\typeout{citep}
  \@ifnextchar[%
  {\citepOpt@i}%<- if next char is '[', we call the version that processes optional arguments
  {\citepNoOpt}%   %<- else we call cite
}

\def\citepNoOpt#1{%
  %\typeout{citepNoOpt called with '#1'}
  {\cite{#1}}%
}

\def\citepOpt@i[#1]{%  
  %\typeout{citepOpt@i  called with '#1' }
  \@ifnextchar[%
  {\citepOpt@ii{#1}}%<- if next char is '[', we call the version that processes 2 optional arguments
  {\citepOneOpt{#1}}%<- else we call cite with 1 optional argument
}
\def\citepOneOpt#1#2{%
  %\typeout{citepOneOpt called with '#1' '#2'}
  \cite[#1]{#2}%
}
\def\citepOpt@ii#1[#2]#3{%
  %\typeout{citepOpt@i  called with '#1' '#2' '#3'}
  {\ifempty{#2} 
      {\cite<#1>{#3}}
  \else
      {\cite<#1>[#2]{#3}}
  \fi}%
}

\makeatother
\newcommand{\citet}[2][]{{\ifempty{#1}\citeA{#2}\else\citeA[#1]{#2}\fi}}
\newcommand{\citealp}[2][]{{\ifempty{#1}\citeR{#2}\else\citeR[#1]{#2}\fi}}
\newcommand{\citealt}[2][]{{\ifempty{#1}\citeR{#2}\else\citeR[#1]{#2}\fi}}


